An Improved Semi-Supervised VAE for Learning Disentangled Representations

Learning interpretable and disentangled representations is a crucial yet challenging task in representation learning. In this work, we focus on semi-supervised disentanglement learning and extend work by Locatello et al. (2019) by introducing another source of supervision that we denote as label replacement. Specifically, during training, we replace the inferred representation associated with a data point with its ground-truth representation whenever it is available. Our extension is theoretically inspired by our proposed general framework of semi-supervised disentanglement learning in the context of VAEs which naturally motivates the supervised terms commonly used in existing semi-supervised VAEs (but not for disentanglement learning). Extensive experiments on synthetic and real datasets demonstrate both quantitatively and qualitatively the ability of our extension to significantly and consistently improve disentanglement with very limited supervision.

==> content/model_plot.tex <==

\begin{figure}[t]
\centering

\tikzstyle{encoder}=[trapezium,
            thick,
            trapezium angle=70, 
            inner ysep=2mm,
            inner xsep=2.5mm,
            draw=black,
            ]
            
\tikzstyle{decoder}=[trapezium,
            thick,
            trapezium angle=70, 
            inner ysep=2mm,
            inner xsep=2.5mm,
            draw=black,
            rotate=180,
            ]

\begin{tikzpicture}[>=latex,text height=1.5ex,text depth=0.25ex]

\matrix[row sep=6mm,column sep=0cm] {
    & & \node (x') {$\widehat{\vx}$}; &  & &[6ex] & \node (y1') {\color{PineGreen}$\widehat{\vy}_1$}; &[-2ex]
    \node (z1) {\color{blue}$\widehat{\vz}_1$}; &[-1ex] &[-1ex]
    \node (z2) {\color{blue}$\widehat{\vz}_2$}; &[-2ex]
    \node (y2') {\color{PineGreen}$\widehat{\vy}_2$}; \\
    & & \node (dec) [decoder]{\rotatebox[x=0mm, y=1mm]{180}{Dec}};& & & & \node (enc1) [encoder]{Enc}; & & & &
    \node (enc2) [encoder]{Enc}; \\
    \node (y) {\color{red} $\vy$}; & & \node (y') {\color{red} $\widehat{\vy}$}; & & \node (z) {$\widehat{\vz}$}; & &
    \node (x1) {$\widehat{\vx}_1$}; & & & &
    \node (x2) {$\widehat{\vx}_2$}; \\
    & & \node (enc) [encoder]{Enc}; & & & &
    \node (dec1) [decoder]{\rotatebox[x=0mm, y=1mm]{180}{Dec}}; & & & &
    \node (dec2) [decoder]{\rotatebox[x=0mm, y=1mm]{180}{Dec}}; \\
     & & \node (x) {$\vx$};
    & & 
     & &
    \node (y1) {\color{PineGreen}$\vy_1$}; & & 
    \node (z') {$\vz$}; & & 
    \node (y2) {\color{PineGreen} $\vy_2$}; & & \\[-10pt]
    & & \node (lab_a) {(a)}; & & & & & & \node (lab_b) {(b)}; \\
};

\path[->]
(x) edge[thick] (enc)
(enc) edge[thick] (y')
(enc) edge[thick] (z)
(y) edge[thick, dashed] (dec)
(y') edge[thick] (dec)
(z) edge[thick, dashed] (dec)
(y1) edge[thick] (dec1)
(z') edge[thick] (dec1)
(z') edge[thick] (dec2)
(y2) edge[thick] (dec2)
(dec1) edge[thick] (x1)
(dec2) edge[thick] (x2)
(x1) edge[thick] (enc1)
(x2) edge[thick] (enc2)
(enc1) edge[thick] (y1')
(enc1) edge[thick] (z1)
(enc2) edge[thick] (z2)
(enc2) edge[thick] (y2')
;

\path (dec.north east) -- (dec.north) coordinate[pos=2.2] (a1);
\path (z.north east) -- (z.north) coordinate[pos=1.3] (b1);
\draw[-latex, thick] (b1) -- (a1);

\path (dec.south east) -- (dec.south) coordinate[pos=1.2] (a2);
\path (x'.south east) -- (x'.south) coordinate[pos=0.7] (b2);
\draw[-latex, thick] (a2) -- (b2);

\path (dec.south west) -- (dec.south) coordinate[pos=1.25] (a3);
\path (x'.south west) -- (x'.south) coordinate[pos=0.6] (b3);
\draw[-latex, thick, dashed] (a3) -- (b3);


\end{tikzpicture}
\vspace{-3mm}
\caption{
Illustration of our proposed method. (a) shows the standard VAE forward pass with label replacement when supervision is available. (b) shows the reverse pass that attempts to maximize the mutual information between factor code and input image and at the same time minimize the information contained in the nuisance code $\vz$. The loss terms in addition to standard VAEs are marked with color. Red denotes label loss, blue denotes inconsistency minimization loss and green denotes mutual information maximization loss. Best viewed in color.}
\label{model}
\end{figure}
